Memory-Based Semantic Parsing

We present a memory-based model for context-dependent semantic parsing. Previous approaches focus on enabling the decoder to copy or modify the parse from the previous utterance, assuming there is a dependency between the current and previous parses. In this work, we propose to represent contextual information using an external memory. We learn a context memory controller that manages the memory by maintaining the cumulative meaning of sequential user utterances. We evaluate our approach on three semantic parsing benchmarks. Experimental results show that our model can better process context-dependent information and demonstrates improved performance without using task-specific decoders.

==> 10_response.tex <==
\section{Response to reviews}
We thank the reviewers for their thorough feedback and their
suggestions regarding our baseline experiments, claims, and
analysis. We summarize below the changes we made:
\begin{itemize}
\item As suggested, we submitted our model to the Sparc and Cosql
  leader-boards and added the numbers in
  Table~\ref{tab:sparc_result}. We do not report test results for base
  models as we are not allowed to make multiple submissions according
  to  leader-board rules. However,  development
  set results correlate with test set results which allows us to
  compare models and draw further conclusions. 


\item With regard to using a simpler seq2seq baseline which
  concatenates the previous utterances, both
  Table~\ref{tab:atis_result} and~\ref{tab:sparc_result} have this
  baseline. For ATIS, Seq2Seq+concat in Table~\ref{tab:atis_result}
  corresponds to this setting. For SparC and CoSQL, CDS2S in
  Table~\ref{tab:sparc_result} also concatenates the previous
  utterances.

\item For ATIS, we have also added another baseline HE-LSTM based on
  \citet{suhr-etal-2018-learning}.

\item To measure the effectiveness of chunk merging, reviewers
  suggested an experiment where we do not use sentence chunking and
  instead used tokens as phrases. We retrained our model (Mem-LSTM in
  Table~\ref{tab:atis_result}), and tuned hyperparameters in a similar
  manner as mentioned in Section~\ref{sec:experimental-setup}. We
  observed a significant decrease in performance with 34.3\%
  denotation accuracy. The same model with chunk merging achieves
  63.3\% denotation accuracy. We have not reported these experiments
  in the paper due to lack of space, but could incorporate them if we
  are given a bit more space.

\item In order to add a grammar-based decoder for the ATIS dataset, we
  contacted the authors of \url{https://arxiv.org/pdf/1905.13326.pdf}
  for their model configuration (the model is implemented as part of
  the AllenNLP~\footnote{https://allennlp.org/} toolkit). However,
  despite best efforts, we were unable to reproduce their
  results. Nevertheless, with their best model configuration and our
  memory-based interaction encoder, we obtained 55\% denotation
  accuracy compared to 53.2\% with a base model (using the same
  hyperparameters). We did not report these results in the main paper,
  since a different decoding method is slightly orthogonal to our
  contribution.

\item We experimented with a reset mechanism to handle stale content
  which might be helpful for longer interactions as those seen in
  ATIS. Specifically, we propose to learn a context reset
  classifier. Based on the current utterance, the classifier can
  decide if it is context independent in order to erase the memory and
  start a new context. For utterance hidden representation~$h_{i}^U$,
  the reset probability is:
    \begin{equation*}
        \beta = \sigma(W^{r'}(\operatorname{ReLU}(W^r h_{i}^U + b^r) + b^{r'}))
    \end{equation*}
    We then use $\beta$ to reset context as,
    \begin{equation*}
        M_i^t = (1 - \beta) M_i^{t - 1}
    \end{equation*}
    However, we found that this made learning harder without improving
    performance. Manual inspection showed that the learned behaviour
    was not expected or explainable. We thank the reviewer for this
    suggestion and plan to address learning stability issues in future
    work.

  \item We added Table~\ref{tab:analysis} which extends our analysis
    on the ATIS dev set subsample. We retrained the model proposed by
    \citet{suhr-etal-2018-learning} using the code available at
    \url{https://github.com/lil-lab/atis} and computed statistics on
    our annotated sample for comparison.

  \item In general, we have fixed writeup issues highlighted by the
    reviewers and updated our claims to be more aligned with our
    results.
\end{itemize}
For our experiments on SparC and CoSQL, we selected models which were
open-source and state-of-the-art at the time of submission. Please
note that the dates on the leader-board only reflect the release date
of the scores and not when the paper or code is released.
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "tacl2018v2-template"
%%% End: 


==> 5_1_mem_plot.tex <==
\setlength\dashlinedash{0.4pt}
\setlength\dashlinegap{1.5pt}
\setlength\arrayrulewidth{0.3pt}

\renewcommand{\arraystretch}{1.5}
%https://tex.stackexchange.com/questions/40561/table-with-multiple-lines-in-some-cells
\begin{figure*}[ht]
%\centering
%\resizebox{\textwidth}{!}{%
\small
%\begin{tabular}{|l|p{0.12\textwidth}|p{0.12\textwidth}|p{0.12\textwidth}|p{0.12\textwidth}|p{0.12\textwidth}|p{0.12\textwidth}|p{0.12\textwidth}|}
%\begin{tabular}{|L|L|L|L|L|L|L|L|}
\begin{tabularx}{\textwidth}{| l | X | X | X | X | X | X | X | }\hline
 \parbox[t]{4mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\#Memory Slot}}} &
\textit{Q1: Continental airlines on 1993 February twenty Seventh from Chicago to Seattle} &
\textit{Q2: Show 1993 February twenty eighth flights from Seattle to Chicago} &
\textit{Q3: Only flights after 1700 hours} &
\textit{Q4: Only flights after 1700 hours} &
\textit{Q5: Only flights after 1500 hours} &
\textit{Q6: Show all 1993 February twenty eighth flights on Continental} &
\textit{Q7: Only those on Continental airlines}
 \\ \midrule 
 0 &
 Continental airlines & 
 \hlb{Continental airlines} & 
 \hlpink{Only flights} & 
 Only flights & 
 Only flights & 
 Only flights &
 Only those 
 \\ \hdashline
 1 &
 \textbf{on} 1993 February twenty \textbf{seventh} & 
 \textbf{Show} 1993 February twenty \textbf{eighth} flights & 
 Show 1993 February twenty eighth flights & 
 Show 1993 February twenty eighth flights & 
 Show 1993 February twenty eighth flights & 
 \textbf{Show all} 1993 February twenty eighth flights & 
 Show all 1993 February twenty eighth flights 
 \\ \hdashline
 2 &
 from Chicago & 
 from Seattle & 
 from Seattle & 
 from Seattle & 
 from Seattle & 
 \textit{from Seattle} & 
 from Seattle
 \\ \hdashline
 3 &
 to Seattle & 
 to Chicago & 
 to Chicago & 
 to Chicago & 
 to Chicago & 
 \textit{to Chicago} & 
 to Chicago
 \\ \hdashline
 14 &
 - & 
 - & 
 after 1700 hours & 
 after 1700 hours & 
 after \textbf{1500} hours & 
 \hlb{after 1500 hours} & 
  \hlb{after 1500 hours}
 \\ \hdashline
 15 &
 - & 
 - & 
 - & 
 - & 
 - & 
 on Continental & 
 on Continental 
 \\ \hline
& \ding{51} & \ding{55} &  \ding{51} &  \ding{51} &  \ding{51} &  \ding{55} & \ding{55}
\\  \hline
\end{tabularx}
%} %resize
\caption{Memory plot with max. Correct(\ding{51}) / Incorrect(\ding{55}). \fcolorbox{black}{lightblue}{\rule{0pt}{6pt}\rule{6pt}{0pt}}: Stale content in memory w.r.t the current utterance. \fcolorbox{black}{pink}{\rule{0pt}{6pt}\rule{6pt}{0pt}}: Incorrect substitution.}
\label{mem-plot}
\end{figure*}

